Towards a Wearable Interface for Food Quality Grading through ERP Analysis

Sensory evaluation is used to assess the consumer acceptance of foods or other consumer products, so as to improve industrial processes and marketing strategies. The procedures currently involved are time-consuming because they require a statistical approach from measurements and feedback reports from a wide set of evaluators under a well-established measurement setup. In this paper, we propose to collect directly the signal of the perceived quality of the food from Event-related potentials (ERPs) that are the outcome of the processing of visual stimuli. This permits to narrow the number of evaluators since errors related to psychological factors are by-passed. We present the design of a wearable system for ERP measurement and we present preliminary results on the use of ERP to give a quantitative measure to the appearance of a food product. The system is developed to be wearable and our experiments demonstrate that is possible to use it to identify and classify the grade of acceptance of the food.

==> content/old_introrelated.tex <==
%% main text
\section{Introduction}

During the last years, technology enhancement has enabled several technique for addressing fatigue monitoring and drowsiness detection. Automotive industry is proposing solutions based on the use of on-board vehicle sensors to monitor and prevent dangerous situations, making the vehicle \textit{smarter}. Other systems focus on the physical behavior on the the driver to determine drowsiness. By using on-board cameras, eye and face tracking systems aim to monitor driver’s eye parameters as PERCLOS (percent of time with eyelid closed at least 80 \%, measured in a minute) \cite{5625960}, eye blink ratio or the yawning occurrence. Latety, the duration of the blink has been taken as an important parameter to determine drowsiness \cite{Caffier2003}, \cite{SUGIYAMA1996159}. Nevertheless, a wide applicability of them is not possible since they are functional in specific conditions. Cockpit cameras require to have a clear line of sight and a good alignment.

The monitoring of the physiological parameters, which represents the leading causes of reduced attention, permits a more direct way to detect fatigue and drowsiness and it was widely studied in scientific literature \cite{kokonozi2008study, 5580017, yang2010driver}. The analysis of EEG (Electroencephalography) signals is the most commonly used method to detect the drowsiness.
The energy level of the alpha waves (8-13 Hz) and theta waves (4-8 Hz) proven to be good indicators of drowsiness according previous researches (cite). These indicators can be used to automatically recognize the drowsiness in real time. 

Taking this in consideration, in this work, a system to provide drowsiness alerts was developed using only the information coming from the EEG signals. This relays in three different level of alarms. The first considers the blink duration, taken from the EEG eye-blink artifacts,  to provide an early alert since the increase of the blink duration have been proven to be a good indicator of drowsines [cita]. The second level is coming from the presence of small busts of alpha waves. These can be present in drowsy conditions as it was proven by previous investigations. The third level, also related to the presence of alpha waves, indicates the total closure of the eyes by considering the constant presence of alpha waves for a given time. The system was validated on 7 test subject achieving an average accuracy of 83\%. Thanks to the use of a single electrode configuration, this implementation aims to replace the use of cameras in order to have a fully wearable device. 

\section{Related Work}

% very basics commercial approaches


Although these monitoring techniques have proven to be continuous, non-intrusive, and cost-effective, a new trend of research is to couple them with systems that can measure of physical changes during fatigue such as computer vision (PERCLOS, Blink Frequency, Blink duration, Nodding and Yawing occurrences). Still, computer vision analysis results to be difficult task, even for humans, because there are many factors involved, for instance, changing illumination conditions and a variety of possible facial postures. For example, Flores et. al. \cite{FloresJASP2010} couples a digital camera to compute the driver’s eye state and eye blinking frequency, head movement and sagging body posture that operates accurately in daily lightning conditions. For nocturnal conditions, the use NIR (near infra red) illumination and stereo vision has been proven to provide better performance \cite{JiTCT2004}, \cite{KolliINDS2011}. Thus, these different conditions are forcing the implementation of more complex hardware and software. 

To overcome these issues, and to provide a more direct approach to detect drivers drowsiness, the new approach consist in directly measure biometrical signals such as EEG , EOG (Electrooculography),  ECG, PPG (Photoplethysmogram),  and eventually fusing data \cite{KhaleghiIF2011}\cite{GravinaIF2016} to improve the robustness of the approach \cite{SathyanarayanaIF2010}. Few of these approaches have been prototyped and demonstrated in practical driving applications. Shin et. al \cite{ShinSENSORS2010} proposed a system for drowsiness detection based on an ECG sensor with and PPG (Photoplethysmogram) to monitor health conditions of the driver. Reyes et. al.\cite{ReyesSENSORS2016} proposed the integration of body sensor networks and vehicular ad-hoc networks for traffic safety. Thanks to the lower computational requirement of this direct measurement with respect to computer vision, it's possible to reduce the required hardware to low-power microcontrollers, to achieve portability. 

The current work it is inspired by the new trend on wearable devices, using a reduced hardware configuration. The systems scans the EEG signals to extract well-known behavioral and physiological parameters. During the development of the project, several indicators were evaluated for this purpose. Finally, the blink duration and the presence of alpha waves were selected to elaborate a three-level drowsiness detector system. The extraction of the features is purely based on power spectrum techniques.  The system validation was done with 7 test subject, performing controlled simulated actions. The final average accuracy detection of the three level of alarms was of 83\%


%The first level, that keeps track on the blink duration, aims to give an early alert about fatigue. This is done extracting information from the eye-blink artifacts present on EEG. For this, the power spectrum of lower frequencies is analyzed with the aim to separate parameters that are not of interest (saccades, fast blinks, other artifacts). The second level relies on the presence of alpha waves. According {}, small burst of alpha waves can detected while drowsiness conditions are present, specially when performing long blinks ( \textgreater 500 ms). The first and the second levels of alarm are evaluated in a time window of 20 seconds to a given threshold to provide the alarms, following the techniques used in other researches with large datasets.  The third level of alarm considers also the level of energy of the alpha waves, but in this case without any window. This provides a shortcut to inform as soon is possible about the imminent closure of the eyes. This is possible due to the well documented relation with the closure of the eyes and the production of alpha waves (cita), (cita).

%%add the battery thing.
